Residual path integrals for re-rendering

Conventional rendering techniques are primarily designed and optimized for single-frame rendering. In practical applications, such as scene editing and animation rendering, users frequently encounter scenes where only a small portion is modified between consecutive frames. In this paper, we develop a novel approach to incremental re-rendering of scenes with dynamic objects, where only a small part of a scene moves from one frame to the next. We formulate the difference (or residual) in the image between two frames as a (correlated) light-transport integral which we call the residual path integral. Efficient numerical solution of this integral then involves (1)~devising importance sampling strategies to focus on paths with non-zero residual-transport contributions and (2)~choosing appropriate mappings between the native path spaces of the two frames. We introduce a set of path importance sampling strategies that trace from the moving object(s) which are the sources of residual energy. We explore path mapping strategies that generalize those from gradient-domain path tracing to our importance sampling techniques specially for dynamic scenes. Additionally, our formulation can be applied to material editing as a simpler special case. We demonstrate speed-ups over previous correlated sampling of path differences and over rendering the new frame independently. Our formulation brings new insights into the re-rendering problem and paves the way for devising new types of sampling techniques and path mappings with different trade-offs.

==> latexmkrc <==
#!/usr/bin/perl

## Put this (Perl) file in the root of your Overleaf project. It overrides the
## `pdflatex` compilation command to run GhostScript as a post-process which will
## compress non-JPEG images to JPEG in the output PDF file. The JPEG quality
## settings are set to high to minimize the loss of image quality. This should
## work well even for images that contain a lot of high-frequency noise.
## To disable, simply rename the file to something other than latexmkrc.
##
## Created by Iliyan Georgiev.

## Quality settings
$PDF_VERSION = 1.4;
$IMG_DOWNSAMPLE = 'true';
$IMG_DOWNSAMPLE_DPI = 600;
$IMG_DOWNSAMPLE_THRESHOLD = 1.0;
$IMG_COMPRESSION_QFACTOR = 0.15;  # lower is better (try 0.08 for higher quality)
$PASSTHROUGH_JPEGS = 'true';

## Don't modify these, they are specified by Overleaf
$GS_INPUT_FILE = '%B.pdf';
$GS_OUTPUT_FILE = '%B-embed.pdf';

## You can try setting below: -dNEWPDF=true
## This fails in the current GhostScript v9.55 on Overleaf 
$GS_COMMAND = "gs
   -sDEVICE=pdfwrite
   -sOutputFile=$GS_OUTPUT_FILE
   -dCompatibilityLevel=$PDF_VERSION
   -dPDFSETTINGS=/default
   -dFastWebView=true
   -dEmbedAllFonts=true
   -dSubsetFonts=true
   -dCompressFonts=true
   -dDetectDuplicateImages=true
   -dDoThumbnails=false
   -dAutoRotatePages=/None
   -dDownsampleColorImages=$IMG_DOWNSAMPLE
   -dColorImageDownsampleType=/Bicubic
   -dColorImageDownsampleThreshold=$IMG_DOWNSAMPLE_THRESHOLD
   -dColorImageResolution=$IMG_DOWNSAMPLE_DPI
   -dDownsampleGrayImages=$IMG_DOWNSAMPLE
   -dGrayImageDownsampleType=/Bicubic
   -dGrayImageDownsampleThreshold=$IMG_DOWNSAMPLE_THRESHOLD
   -dGrayImageResolution=$IMG_DOWNSAMPLE_DPI
   -dDownsampleMonoImages=$IMG_DOWNSAMPLE
   -dMonoImageDownsampleType=/Subsample
   -dMonoImageDownsampleThreshold=$IMG_DOWNSAMPLE_THRESHOLD
   -dMonoImageResolution=$IMG_DOWNSAMPLE_DPI
   -dConvertCMYKImagesToRGB=true
   -dColorImageFilter=/DCTEncode
   -dGrayImageFilter=/DCTEncode
   -dMonoImageFilter=/CCITTFaxEncode
   -dColorConversionStrategy=/LeaveColorUnchanged
   -dPassThroughJPEGImages=$PASSTHROUGH_JPEGS
   -dProcessColorModel=/DeviceRGB
   -dRenderIntent=1
   -dDefaultRenderingIntent=/Perceptual
   -dUseArtBox
   -dNEWPDF=false
   -dNOPAUSE
   -dBATCH
   -c \"<< /ColorACSImageDict << /VSamples [ 1 1 1 1 ] /HSamples [ 1 1 1 1 ] /QFactor $IMG_COMPRESSION_QFACTOR /Blend 1 /ColorTransform 1 >> >> setdistillerparams\"
   -f $GS_INPUT_FILE";

## Remove new-line characters from GhostScript command
$GS_COMMAND =~ s/\n//g;

## Set the pdflatex command to be used by Overleaf
$pdflatex = "pdflatex %O %S; $GS_COMMAND; mv %B-embed.pdf %B.pdf";

## For debugging
# print "$GS_COMMAND\n";
# print "$pdflatex\n";

